CogReact: A Reinforced Framework to Model Human Cognitive Reaction Modulated by Dynamic Intervention

Using deep neural networks as computational models to simulate cognitive process can provide key insights into human behavioral dynamics. Challenges arise when environments are highly dynamic, obscuring stimulus-behavior relationships. However, the majority of current research focuses on simulating human cognitive behaviors under ideal conditions, neglecting the influence of environmental disturbances. We propose CogReact, integrating drift-diffusion with deep reinforcement learning to simulate granular effects of dynamic environmental stimuli on human cognitive process. Quantitatively, it improves cognition modelling by considering temporal effect of environmental stimuli on cognitive process and captures both subject-specific and stimuli-specific behavioural differences. Qualitatively, it captures general trends in human cognitive process under stimuli, better than baselines. Our approach is examined in diverse environmental influences on various cognitive tasks. Overall, it demonstrates a powerful, data-driven methodology to simulate, align with, and understand the vagaries of human cognitive response in dynamic contexts.

==> 6_eval_learning.tex <==
% \section{Evaluation 3: Learning Task}
% The previous cognitive tasks require humans to make discrete choices. We further extend our model into a more general scenario for continuous input, i.e. curiosity, coming from the PeerEdu dataset. This behavior shows most significantly impact due to peer feedback compared with other behaviors in PeerEdu. Therefore, we use this behavior for our exploration.


% \subsection{Simulation Performance}

% We use the same baseline models as experiment 2. Moreover, since both task and feedback are textual input instead of numeric input in experiment 1, we use embeddings extracted from textual data for baseline model input.


% \subsection{Ablation Study}


% Remove LLM learning agent (numeric encoding or string encoding for SVM), Remove DDM (pure RL), remove DDM+RL (pure SVM)

% \subsection{CogReact Better Captures Intervention Effect}




